Learning to Formulate: Agentic Hardware-Software Co-Design of AI Infrastructure through Progressive Optimization and Verification

AI infrastructure, the chips and software that train and serve AI models, is designed in layers. Layers make the system manageable, but they also fix which choices an optimizer can consider. Gains that need the chip and its software to change together are excluded before optimization begins: the formulation leaves them out. Language-model agents make it possible to revisit these boundaries, but an agent's proposal cannot show by itself that a design is correct or optimal. We present Formulaic, a flow that divides the work. The agent writes the formulation, a mathematical solver optimizes within it, and verification and measurement check its assumptions and results. The agent refines the problem step by step, from the computation graph toward the chip. Each step is a template: a family of programs with the conditions under which they are correct. Wall relaxation searches the chip by pricing the hardware limits that bind the software. This paper takes a first step, through separate studies rather than one end-to-end run. On NVIDIA GB10, templates the agent wrote run complete Qwen3-8B layers $1.075\times$ faster than SGLang. In a simulated Ventus GPU study, joint design cuts the worst-scenario cycles of Qwen2.5-0.5B to 0.428 of the reference, against 0.934 for software alone. On a five-step GEMM refinement chain, reusing proofs makes checking $2.51\times$ faster.

==> experiments/latex/format.tex <==
% Load in the preamble of either the standalone manuscript or the full paper.
\RequirePackage{amsmath,amssymb,booktabs,tabularx,array,graphicx,xcolor}
\RequirePackage{placeins,xurl}
\RequirePackage{caption}
\definecolor{experimentmuted}{HTML}{52616B}
\providecommand{\ExperimentRoot}{.}
\providecommand{\ExperimentSection}{\section}
\providecommand{\ExperimentSubsection}{\subsection}
\providecommand{\ExperimentSubsubsection}{\subsubsection}
\providecommand{\us}{\ensuremath{\mu\mathrm{s}}}
\providecommand{\tbd}{\textcolor{experimentmuted}{[TBD]}}
\providecommand{\tnote}[1]{\par\vspace{2pt}{\footnotesize\noindent #1\par}}
\providecommand{\lead}[1]{\par\noindent\textbf{#1}\ }
\providecommand{\ExperimentCitation}[1]{}

